CoolerSpace: A Language for Physically Correct and Computationally Efficient Color Programming

Color programmers manipulate lights, materials, and the resulting colors from light-material interactions. Existing libraries for color programming provide only a thin layer of abstraction around matrix operations. Color programs are, thus, vulnerable to bugs arising from mathematically permissible but physically meaningless matrix computations. Correct implementations are difficult to write and optimize. We introduce CoolerSpace to facilitate physically correct and computationally efficient color programming. CoolerSpace raises the level of abstraction of color programming by allowing programmers to focus on describing the logic of color physics. Correctness and efficiency are handled by CoolerSpace. The type system in CoolerSpace assigns physical meaning and dimensions to user-defined objects. The typing rules permit only legal computations informed by color physics and perception. Along with type checking, CoolerSpace also generates performance-optimized programs using equality saturation. CoolerSpace is implemented as a Python library and compiles to ONNX, a common intermediate representation for tensor computations. CoolerSpace not only prevents common errors in color programming, but also does so without run-time overhead: even unoptimized CoolerSpace programs out-perform existing Python-based color programming systems by up to 5.7 times; our optimizations provide up to an additional 1.4 times speed-up.

==> new-tex/new-limit.tex <==
\section{Limitations}

There are several limitations of \colorlang that we address below. There are some inherent limitations of \colorlang such as the lack of control flow. Other limitations can be addressed with more development.

\paragraph{User-input color spaces.} There are a vast number of color spaces used by industry today. It is not feasible to support every single color space a programmer might want to use. Color spaces are defined by ICC profile files. \colorlang should be extended to allow users to define types from ICC profiles. Implementing this feature would require a re-work of our type system.

\paragraph{Rendering intents.} Currently we do not support rendering intents for images that are converted to \texttt{sRGB} and \texttt{opRGB}. These spaces can only express a finite set of colors. It is possible for colors to be out of the gamut of these two color spaces. In such a scenario, a rendering intent algorithm would be applied to re-map the out-of-gamut colors. Implementing rendering intents would not require significant changes to the type system or syntax of our language. 

\paragraph{Control flow.} We have chosen to implement \colorlang in python for the sake of accessibility. However, since \colorlang is a python library, it is unable to capture the control flow of the user's program. In order to address this problem, \colorlang would have to be re-implemented as its own language. 


==> new-tex/new-pipeline.tex <==
\subsection{Python and Type Checking}

Since Python is useful for rapidly prototyping scientific scripts, it is the default choice for scientists for many application. It is also the de-facto language for color science and related applications. However, since it is dynamically typed, type checking in Python requires either prohibiting certain features of dynamically typed code or utilizing gradual typing methods. 

In \colorlang, we perform dynamic type checks when \colorlang expressions are read by the Python interpreter and captured by our library through operator overloading. We maintain a tree of \colorlang expressions, augmenting it with new operators as they are type checked. This allows us to perform type checks as early as possible while keeping it dynamic like most Python code. We lazily evaluate the values when they are rendered or otherwise accessed by the user, thereby ensuring that expensive computation is not performed if there are type errors later down in the code. 

Of course, dynamic type checking and lazy evaluation adds non-negligible overhead to run-time costs. Our optimization algorithms discussed in the next section can be utilized in a statically typed language, in which case most overhead costs can be completed during compile time. As such, our theoretical contributions reach beyond the practical implementation of \colorlang, which may be less efficient than existing color programming libraries. With that said, in scenarios with high data volume, we show that even with the runtime overhead, our optimizations result in faster runtime than poorly written code. This is an important benefit of \colorlang since it is not uncommon to process millions of pixels in digital imaging. 

\subsection{Interpretation vs Compilation}

After type checking and tree building, it is natural to traverse the expression tree in order to evaluate needed values. We design our pipeline to include compilation rather then stopping at interpretation for several reasons .

First, a statically analyzed variant of our system is a trivial extension. Since we do not employ any type checking rules that can only be done dynamically, our system could be ported to a compiled language with statically determined ndarray dimensions where all type checking could be done in compile-time. The popularity of Python among color scientists is the primary reason why we made concessions in static analysis. 

Second, we aim to study color \& light manipulation expression optimizations in general. Our techniques described in the next subsection could be employed in all programming systems in related domains, whether it be interpreted, compiled, or just-in-time compiled. 

Third, we argue that \colorlang expressions would often be wrapped in a function that could be called many times to batch process many inputs. Compiling an optimized version of a large \colorlang expression could reap repeated runtime benefits. 

\subsection{Target Language}

After type checking, we choose to compile the target expression in order to reap repeated runtime benefits. Our target language of choice is tensor algebra, namely the Open Neural Network Exchange (ONNX) file format commonly used in AI/ML. We choose tensor algebra as our target language for several reasons. 

\begin{enumerate}
    \item Almost all color \& light operations can be naturally reduced to tensor algebra. We show that even more complex operations such as nonlinear color space transformations, gamma mapping, and pigment mixing can be written in ONNX.
    \item Color \& light operations benefit greatly from parallelization in the GPU, which is a similar workflow as neural networks. Existing ONNX runners already employ parallelization and a host of low-level optimization tricks.
    \item Compiling down to tensor algebra allows us to reap the benefits of any advancements in tensor algebra optimization without reinventing the wheel. With the considerable amount of attention in AI/ML, tensor algebra optimizers and runners are likely to improve significantly.
    \item Many downstream tasks also map easily to tensor algebra. For instance, edge detection and gaussian blur both involve convolutions. Thus, while image processing is outside the scope of this paper, it is natural to extend the compiled tensor algebra graph in order to augment the color transformation algorithm with image processing tasks. 
\end{enumerate}

While the ONNX file format is suitable for executing tensor algebra, its serialized nature makes it not suitable for use in theoretical discussions and in the equality saturation phase of our pipeline. Thus, we describe \textsc{TnsrLang}, a lisp-like tensor algebra language that is modelled after TENSAT. \textsc{TnsrLang} implements a subset of tensor algebra operators available in ONNX. It contains fewer operators than TENSAT since we do not need ML operators that do not appear in color science. On the other hand, we also extend TENSAT to include the scalar power operator, which is used for nonlinear color space transformations and gamma mapping. The full list of operators in \textsc{TnsrLang} is described below. 

\begin{table}[!htb]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Operator & Description & Type Signature \\
        \hline
        input & input tensor & $Str \to T$ \\
        input & input scalar & $Str \to S$ \\
        Mul & element-wise multiplication & $(T, T) \to T$ \\
        Div & element-wise division & $(T, T) \to T$ \\
        Add & element-wise addition & $(T, T) \to T$ \\
        Neg & element-wise negative & $T \to T$\\
        Sub & element-wise subtraction & $(T, T) \to T$\\
        Matmul & element-wise multiplication & $(T, T) \to T$ \\
        Relu & relu activation & $T \to T$ \\
        transpose & matrix transpose & $(T, S) \to T$ \\
        Pow & element-wise exponentiation & $(T, N) \to T$ \\
        Pow & tensor exponentiation & $(T, T) \to T$\\
        Transpose & transpose & $T \to T$\\
        noop & combine multiple outputs & $(T, T) \to T$\\
        smul & scalar multiplication & $(S, T) \to T$\\
        fmul & floating point multiplication & $(S, S) \to S$\\
        fadd & floating point addition & $(S, S) \to S$\\
        \hline
    \end{tabular}
    \caption{Subset of Tensor Algebra Used}
    \label{tab:tensor-algebra}
\end{table}

Input and Pow operators are overloaded such that inputs of tensors and scalars, as well as taking the power of a tensor by a scalar or a tensor (elementwise) are both supported. The input operator take in a string representation of a floating point number or a string of form $\text{name@[T/F]@dim1\_dim2\_}\ldots$. Here "name" is the name of the tensor, "T" or "F" is a boolean that represents whether the tensor is a constant or a variable, and "dim1\_dim2\_\ldots" is a string representation of the tensor's dimensions. 

Next, we describe how \colorlang expressions are converted to \textsc{TnsrLang}. Trivially, any constant or variable object is replaced with ``var\_name@[T/F]@dim1\_dim2\_...". Matrix multiplication or elementwise multiplication between a \colorlang object and a numpy ndarray is natural to translate to tensor algebra. 



\subsection{Optimization Concerns}

Many color \& light operations involve high-resolution images or videos. As such, poorly written expressions can be highly inefficient compared to their more efficient variants. As an elementary example, suppose a programmer wants to take a 4k image in color space $X_1$ and wants to apply a series of linear color space transformations to $X_2, X_3, \ldots, X_k$. Evaluating the expression naively from left to right would involve excessive amount of floating point multiplications. A more efficient method would be to collapse the color space transformation matrices into a single constant matrix. 

In general, optimal high-level optimization of a \colorlang program requires a bag of tricks including constant folding, matrix multiplication reordering, and substitution of sub-expressions into equivalent sub-expressions using arithmetic identities. Traditional optimizers, such as the official `onnx-optimizer`, is based on sequential, greedy passes. As such, they may make bad substitutions with no ability to undo the change. Furthermore, the official \textsc{onnx-optimizer} and others are tailored for the neural network domain. As such, their substitution passes focus on convolutions, kernal mapping, etc., while skimping on optimizations that are applicable most commonly in color science, such as matrix multiplication reordering and bringing the high-resolution image to later down in the execution graph. 

In order to achieve principled high-level optimization on tensor algebra, we extend TENSAT, the state-of-the-art tensor algebra optimizer based on the equality saturation technique. Equality saturation is a method of efficiently maintaining a graph of equivalences between expressions by using e-graphs. Equality saturation still incurs exponential worst-case time since it is a NP-Complete problem. Still, equality saturation allows the optimizer to try many substitutions before extracting a good execution plan, thereby improving the quality of the output graph in practice. Our extension of TENSAT is as follows. First, we add operators such as elementwise power which are required for color science operations, and is part of the ONNX spec. Second, we perform constant folding, which means that graphs that cluster constant tensors together are preferred in the extraction phase. 

\subsection{Pipeline}

Our entire \colorlang compilation pipeline is as follows. First, our \colorlang interpreter dynamically builds an AST of the Python program while performing type-checking in tree-build time. Computation is lazily deferred to later. Then, a \colorlang to ONNX translater takes the AST and outputs an ONNX file. At this point, any ONNX runner can take the file and output a NumPy ndarray. We augment the official \textsc{onnx-optimizer} by running the ONNX file through a standalone ONNX optimizer written in egg, the same equality saturation library that TENSAT uses. Only after the equality saturation do we run our program through \textsc{onnx-optimizer} which performs remaining optimization passes such as constant folding of adjacent constant matrices. After all high-level optimizations are complete, we pipeline the ONNX program to \textsc{onnx-runner} which automatically performs parallel execution with GPUs where possible. 



==> new-tex/new-subrules.tex <==
\begin{enumerate}
    \item INCLUDE: Graphic of implemented substitution rules
    \item Contrast our substitution rules with that of TENSAT. Explain why our substitution rules differ.
\end{enumerate}
